A Unifying Post-Processing Framework for Multi-Objective Learn-to-Defer Problems

Learn-to-Defer is a paradigm that enables learning algorithms to work not in isolation but as a team with human experts. In this paradigm, we permit the system to defer a subset of its tasks to the expert. Although there are currently systems that follow this paradigm and are designed to optimize the accuracy of the final human-AI team, the general methodology for developing such systems under a set of constraints (e.g., algorithmic fairness, expert intervention budget, defer of anomaly, etc.) remains largely unexplored. In this paper, using a $d$-dimensional generalization to the fundamental lemma of Neyman and Pearson (d-GNP), we obtain the Bayes optimal solution for learn-to-defer systems under various constraints. Furthermore, we design a generalizable algorithm to estimate that solution and apply this algorithm to the COMPAS and ACSIncome datasets. Our algorithm shows improvements in terms of constraint violation over a set of baselines.

==> sections/flowchart.tex <==
\begin{tikzpicture}[node distance=1.5cm, auto, font=\small]

% Styles
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3.5cm, minimum height=1cm, text centered, draw=black, fill=red!30]
\tikzstyle{process} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
\tikzstyle{data} = [rectangle, rounded corners, minimum width=3.5cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{arrow} = [thick,->,>=stealth]

% Nodes
\node (start) [startstop, text width=4.5cm] {$\sup_{h, r} \Ebb[L_{def}(h(x), r(x))]$ \\ $\text{ s.t. } \Ebb[\Psi_i(x, h(x), r(x))] \leq \delta_i$};
\node (psi_0) [process, right of=start, xshift=3.25cm, text width=2.5cm] {$\psi_0(x)$ \\ $\text{formula~} \eqref{eqn: psix}$};
\node (estimate_psi_0) [process, right of=psi_0, xshift=2cm, text width=2.5cm] {Estimate $\widetilde{\psi}_0(x)$};
\node (psi_dots) [below of=psi_0, yshift=.5cm] {$\vdots$};
\node (psi_m_plus_1) [process, below of=psi_dots, yshift=.5cm, text width=2.5cm] {$\psi_{m+1}(x)$ \\ $\text{formula~} \eqref{eqn: def_ldefvec}$};
\node (estimate_psi_m_plus_1) [process, right of=psi_m_plus_1, xshift=2cm, text width=2.5cm] {Estimate $\widetilde{\psi}_{m+1}(x)$};
\node (fine_tune) at (5.75, -3.35)[process, xshift=2cm, text width=2.5cm] {Fine tune $k_1, \ldots, k_m$};
\node (fine_tune) at (5.75, -3.35)[process, xshift=2cm, text width=2.5cm] {Fine tune $k_1, \ldots, k_m$};

% New Data Node
\node (data) [ above of=psi_dots, yshift=1.25cm] {$\Dcal_{\mathrm{train}}$};
\node (data_val) [ below of=fine_tune, yshift=0.0cm] {$\Dcal_{\mathrm{val}}$};

% Arrows
\draw [arrow] (start.east) -- ++(0.5,0) |- (psi_0.west);
\draw [arrow] (psi_0) -- (estimate_psi_0);
\draw [arrow] (psi_m_plus_1) -- (estimate_psi_m_plus_1);
\draw [arrow] (start.east) -- ++(0.5,0) |- (psi_m_plus_1.west);
\draw [arrow] (data.south) -- ++(0,-0.5) -- ++(1.75, 0) -- ++(0, -0.7)  -- ++(0.37, 0);
\draw [arrow] (data.south) -- ++(0,-0.5) -- ++(1.75, 0) -- ++(0, -2.7)   -- ++(0.37, 0);
\draw [arrow] (psi_0.east) -- (estimate_psi_0.west);
\draw [arrow] (psi_m_plus_1.east) -- (estimate_psi_m_plus_1.west);
\draw [arrow] (estimate_psi_0.east) -- ++ ( 0.5, 0) --++ ( 0, -3.5) --++ (-1, 0);
\draw [arrow] (estimate_psi_m_plus_1.east) -- ++ ( 0.3, 0) --++ ( 0, -1.25) --++ (-.8, 0);
\draw [arrow] (data_val.north) --++ (0, 0.75);

% Annotations
\node[above of=start, yshift=-1cm] (start_text) {};

\end{tikzpicture}


==> sections/histogram.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{brown}{RGB}{165,42,42}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{paleturquoise}{RGB}{175,238,238}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Normalized Singularity Dimensions },
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Density of dimensions},
ymin=0, ymax=5.67753689897313,
ytick style={color=black}
]
\draw[draw=black,fill=paleturquoise,opacity=0.3] (axis cs:0.340327017994275,0) rectangle (axis cs:0.9085381267712,1.75990927412965);
\addlegendimage{ybar,ybar legend,draw=black,fill=paleturquoise,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=12$}

\draw[draw=black,fill=violet,opacity=0.3] (axis cs:0.427076011175366,0) rectangle (axis cs:0.795005216492022,2.71791416813285);
\addlegendimage{ybar,ybar legend,draw=black,fill=violet,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=32$}

\draw[draw=black,fill=brown,opacity=0.3] (axis cs:0.472385336285866,0) rectangle (axis cs:0.739861681709806,3.73864835940926);
\addlegendimage{ybar,ybar legend,draw=black,fill=brown,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=62$}

\draw[draw=none,fill=paleturquoise] (axis cs:0.00999999999999999,0) rectangle (axis cs:0.0366666666666667,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=paleturquoise}
\addlegendentry{n=12}

\draw[draw=none,fill=paleturquoise] (axis cs:0.11,0) rectangle (axis cs:0.136666666666667,0);
\draw[draw=none,fill=paleturquoise] (axis cs:0.21,0) rectangle (axis cs:0.236666666666667,0.00329089829952167);
\draw[draw=none,fill=paleturquoise] (axis cs:0.31,0) rectangle (axis cs:0.336666666666667,0.0271499109710538);
\draw[draw=none,fill=paleturquoise] (axis cs:0.41,0) rectangle (axis cs:0.436666666666667,0.135749554855269);
\draw[draw=none,fill=paleturquoise] (axis cs:0.51,0) rectangle (axis cs:0.536666666666667,1.55772614196421);
\draw[draw=none,fill=paleturquoise] (axis cs:0.61,0) rectangle (axis cs:0.636666666666667,1.92424994007344);
\draw[draw=none,fill=paleturquoise] (axis cs:0.71,0) rectangle (axis cs:0.736666666666667,2.47403563723728);
\draw[draw=none,fill=paleturquoise] (axis cs:0.81,0) rectangle (axis cs:0.836666666666667,2.31940840990995);
\draw[draw=none,fill=paleturquoise] (axis cs:0.91,0) rectangle (axis cs:0.936666666666667,1.55838950668929);
\draw[draw=none,fill=violet] (axis cs:0.0366666666666667,0) rectangle (axis cs:0.0633333333333333,8.85460824262447e-11);
\addlegendimage{ybar,ybar legend,draw=none,fill=violet}
\addlegendentry{n=32}

\draw[draw=none,fill=violet] (axis cs:0.136666666666667,0) rectangle (axis cs:0.163333333333333,3.68763995589474e-07);
\draw[draw=none,fill=violet] (axis cs:0.236666666666667,0) rectangle (axis cs:0.263333333333333,0.000127949268965153);
\draw[draw=none,fill=violet] (axis cs:0.336666666666667,0) rectangle (axis cs:0.363333333333333,0.00934892313536575);
\draw[draw=none,fill=violet] (axis cs:0.436666666666667,0) rectangle (axis cs:0.463333333333333,0.199342643069134);
\draw[draw=none,fill=violet] (axis cs:0.536666666666667,0) rectangle (axis cs:0.563333333333333,2.46739412419151);
\draw[draw=none,fill=violet] (axis cs:0.636666666666667,0) rectangle (axis cs:0.663333333333333,4.09086763665561);
\draw[draw=none,fill=violet] (axis cs:0.736666666666667,0) rectangle (axis cs:0.763333333333333,2.65825148135252);
\draw[draw=none,fill=violet] (axis cs:0.836666666666667,0) rectangle (axis cs:0.863333333333333,0.546738206097449);
\draw[draw=none,fill=violet] (axis cs:0.936666666666667,0) rectangle (axis cs:0.963333333333333,0.0279286673769142);
\draw[draw=none,fill=brown] (axis cs:0.0633333333333333,0) rectangle (axis cs:0.09,6.28688806645066e-18);
\addlegendimage{ybar,ybar legend,draw=none,fill=brown}
\addlegendentry{n=62}

\draw[draw=none,fill=brown] (axis cs:0.163333333333333,0) rectangle (axis cs:0.19,1.50485075826079e-11);
\draw[draw=none,fill=brown] (axis cs:0.263333333333333,0) rectangle (axis cs:0.29,4.90686985952763e-07);
\draw[draw=none,fill=brown] (axis cs:0.363333333333333,0) rectangle (axis cs:0.39,0.000834008921574049);
\draw[draw=none,fill=brown] (axis cs:0.463333333333333,0) rectangle (axis cs:0.49,0.126873837069594);
\draw[draw=none,fill=brown] (axis cs:0.563333333333333,0) rectangle (axis cs:0.59,3.1458481432568);
\draw[draw=none,fill=brown] (axis cs:0.663333333333333,0) rectangle (axis cs:0.69,5.40717799902203);
\draw[draw=none,fill=brown] (axis cs:0.763333333333333,0) rectangle (axis cs:0.79,1.28981509054716);
\draw[draw=none,fill=brown] (axis cs:0.863333333333333,0) rectangle (axis cs:0.89,0.0294210336618712);
\draw[draw=none,fill=brown] (axis cs:0.963333333333333,0) rectangle (axis cs:0.99,2.93968189345407e-05);
\end{axis}

\end{tikzpicture}

